Visual Servoing in Orchard Settings

We present a general framework for accurate positioning of sensors and end effectors in farm settings using a camera mounted on a robotic manipulator. Our main contribution is a visual servoing approach based on a new and robust feature tracking algorithm. Results from field experiments performed at an apple orchard demonstrate that our approach converges to a given termination criterion even under environmental influences such as strong winds, varying illumination conditions and partial occlusion of the target object. Further, we show experimentally that the system converges to the desired view for a wide range of initial conditions. This approach opens possibilities for new applications such as automated fruit inspection, fruit picking or precise pesticide application.

==> prelim.tex <==
\section{PRELIMINARIES}
\label{sec:pre}

\subsection{Problem Statement}
Let $c_0$ be the initial sensor position approximately $0.5$ m away from the target apple in the workspace $Q \in \mathbb{R}^3$ of the robotic manipulator.
The initial positioning of the manipulator is 


1) a sensor being at position $c_0$ \newline
2) an partially know target in an image at image coordinates $x, y$ with radius $r$ \newline
3) Find and track visual features in the image and minimize the error $e = s - s^*$ until the termination criteria $E = \sum_{i=0}^n e_i^2 < t_h$ is reached \newline

The following assumptions for fruit detections have to hold: \newline
- Apple location $x, y$ is in proximity of center $x_0, y_0$ \newline
- The apple has to be the biggest one as we are focusing on this particular apple which makes $r > r_i$ \newline
- We approximate the apple as a projection of a sphere in the image plane \newline


Do we want to mention here already that we can handle outdoor environment influences?

\vtxt{Unless we do any optimization to decide on the order of fruits, we can formulate the problem for a single fruit. However, instead of the point cloud, can we formulate the input in image coordinates?}


==> standard_includes.tex <==

%% Useful packages
\usepackage{url}
\usepackage{hyperref}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{color}
\usepackage{psfrag}
\usepackage{graphicx,subfigure}
\usepackage{boxedminipage,wrapfig}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{algorithmicx}
\usepackage{multirow}

\usepackage{cite}

%\usepackage[left=1in,top=1in,right=1in,bottom=1in,head=1cm,foot=1cm]{geometry}

%% Useful environment
\newcommand{\mysec}[1]{\vspace{.5cm}\noindent{\bf #1}}
\newcommand{\comment}{\textcolor{blue}}
\newcommand{\vtxt}[1]{\textcolor{red}{V: \textit{{#1}}}}
\newcommand{\degree}{\ensuremath{^\circ}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{case}{Case}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{invariant}{Invariant}
\newtheorem{corollary}{Corollary}
\newcommand{\mat}[1]{{\ensuremath{\mathbf#1}}}
\newcommand{\inv}{{\ensuremath{^{-1}}}}
\newcommand{\transpose}{\ensuremath{^T}}
\newcommand{\expectation}{\ensuremath{\mathbb{E}}}



==> system.tex <==


